A Nonparametric Bayesian Model for Sparse Dynamic Multigraphs

As the availability and importance of temporal interaction data--such as email communication--increases, it becomes increasingly important to understand the underlying structure that underpins these interactions. Often these interactions form a multigraph, where we might have multiple interactions between two entities. Such multigraphs tend to be sparse yet structured, and their distribution often evolves over time. Existing statistical models with interpretable parameters can capture some, but not all, of these properties. We propose a dynamic nonparametric model for interaction multigraphs that combines the sparsity of edge-exchangeable multigraphs with dynamic clustering patterns that tend to reinforce recent behavioral patterns. We show that our method yields improved held-out likelihood over stationary variants, and impressive predictive performance against a range of state-of-the-art dynamic graph models.

==> sections/04_inference.tex <==
\section{Inference}\label{sec:inference}

We provide pseudo-code in Appendix \ref{sec:inference_app}.

\paragraph{Complexity.} The complexity of our model is $O(|E|\times K)$, where $K$ is the number of clusters. The complexity of blockmodel-based models is $O(|V|^2 \times K)$. For sparse graphs, we have $|E| << |V|^2$. In practice, the runtimes of the different models were comparable on the datasets we considered. We note that only hyperparameter sampling uses Metropolis Hastings; the cluster assignments are sampled directly from the posterior conditioned on the hyperparameters.



\iffalse
We perform inference using a sequential Monte Carlo algorithm that approximates the posterior distribution using a swarm of sequentially updated particles \cite{doucet2001introduction}. Using a familiar restaurant analogy, we say that the per-cluster ddCRPs assign senders or recipients of edges to tables, and each table selects a vertex indicator from $H$. Let $b_i^s$ and $b_i^r$ be the table assignments of the $i$th sender and recipient, respectively, and let $\phi_i = (z_i, b_i^{s}, b_i^{r})$ be the set of edge-specific latent parameters for the $i$th edge. Each particle $p$ proposes values for $\phi_i$ according to a proposal distribution $Q(\phi_i^{(p)}|s_i, r_i, \phi_{<i}^{(p)})$, and calculates appropriate importance weights.

In our case, we can analytically evaluate $P(\phi_i^{(p)}|s_i, r_i, \phi_{<i}^{(p)})$, so we use this as our proposal distribution. We can then calculate the importance weights $w_i$ as
$$\begin{aligned}\frac{w_i}{w_{i-1}} \propto& \frac{P(s_i, r_i|\phi_i^{(p)}) pP\phi_i^{(p)}|\phi_{<i}^{
(p)})}{Q(\phi_i^{(p)}|s_i, r_i, \phi_{<i}^{(p)})}\\
=&P(s_i, r_i|\phi^{(p)}_{<i}) .\ \end{aligned}$$
We resample our particles based on the weights $w_i$ whenever the effective sample size drops below 10\% of the number of particles. We include pseudocode and provide analytic expressions for $Q(\phi_i^{(p)}|s_i, r_i, \phi_{<i}^{(p)})$ and $p(s_i, r_i|\phi^{(p)}_{<i})$ in the appendix, and include code with this submission.%\sinead{Check that we're in a position to include code!}

Evaluating the necessary probabilities scales as $O(EK)$, where $E$ is the number of edges and $K$ is the number of clusters. The resampling step adds a cost of $O(P^2)$, where $P$ is the number of particles, making the overall complexity $O(P(EK+P))$. For comparison, the complexity of obtaining $P$ MCMC samples in blockmodel-based  models is $O(PV^2K)$, where $V$ is the number of vertices. For sparse graphs, we have $|E| \ll |V|^2$. %In practice, the runtimes of the different models were comparable on the datasets we considered.\sinead{is this still true?}\elahe{I will check, but shouldn't we provide a proof if we say that?}\sinead{If it is true, I don't think we need to provide proof. Runtime is very much a function of the implementation.}

\fi



==> sections/extras.tex <==

\newpage
\section{New inference}
Each edge is associated with a cluster, $z_i$; a sender-table, $b_i^s$, and a receiver-table, $b_i^r$. These are determined by who the edge follows. The edge has three "following" relationships. $c_i$ is who the $i$th edge cluster-follows -- it determines $z_i$. $g_i^s$ and $g_i^r$ are who the edge sender-follows, and receiver-follows -- they determine the sender-table and the receiver-table.

Note that, an edge can only sender-follow and receiver-follow edges that are in the same cluster! 


\subsection{Sampling the clusters}
We are going to propose a new cluster-follow $c_i^*$, and a new set of sender-follows and receiver-follows $\mathbf{g}^{s*}$ and $\mathbf{g}^{r*}$. We first propose an intermediate ``launch state'' $c_i^\circ, \mathbf{g}^{s\circ},\mathbf{g}^{r\circ}$ (similar to the launch state in the split-merge sampler for the DP):

\begin{itemize}
    \item Let $z_a \leftarrow z_i$
    \item $c_i^\circ = i$
    \item Update $\mathbf{z}^\circ$ to give the launch clusters.
    \item We might now have some edges who sender-follow or receiver-follow an edge that is no longer in the same cluster. Let
    $$\mathcal{M}^s = \{j: z_i^\circ \neq z_{g_i^s}^\circ \}$$
    and
    $$\mathcal{M}^r = \{j: z_i^\circ \neq z_{g_i^r}^\circ \}$$
    \item For every $j \in \mathcal{M}^s$, set $g_j^{s \circ} =j$; for every  $j \not\in \mathcal{M}^s$, set $g_j^{s \circ} =g_j^s$
    \item For every $j \in \mathcal{M}^r$, set $g_j^{r \circ} =j$; for every  $j \not\in \mathcal{M}^s$, set $g_j^{s \circ} =g_j^s$
\end{itemize}


Next, we will sample a proposal $c_i^*, \mathbf{g}^{s*}, \mathbf{g}^{r*}$ from our proposal distribution $q(c_i, \mathbf{g}^s, \mathbf{g}^r) = q(c_i)\prod_{j\in \mathcal{M}^s} q(g_j^s) \prod_{k\in \mathcal{M}^r} q(g_k^r)$. We first sample $c_i^* \sim q(c_i)$ where

$$q(c_i = k) \propto \begin{cases} f_1(d_{ik}) & k<i\\ \alpha & k=i\end{cases}$$

We record $q(c_i)$ and $q(c_i^*)$ (including normalizing constants)

We then update the clusters $\mathbf{z}^*$.

We then sample the sender-tables for $j\in\mathcal{M}^s$

$$q(g_j^s = k) := P(g_j^s = k | z_{\leq j}, g_{<j}^s, s_j) \propto \begin{cases} 
f_2(d_{jk})  & k<j, z^*_i=z^*_k, s_j = s_k \\
\tau h_{s_j} & k=j\\
0 & z^*_i\neq z^*_k\\
0 & s_i \neq s_k \end{cases}$$

and similarly sample the receiver-tables for $j\in\mathcal{M}^r$.

We record $q(g_j^{s*})$ and $q(g_j^{s})$ for each $j\in \mathcal{M}^s$ -- note that the distributions will be different for the original state and the proposed state! Ditto for the receivers.

Now, we need to calculate the MH acceptance ratio. In general, we have an acceptance ratio of

$$\min\left(1, \frac{q(c_i, \mathbf{b}^s, \mathbf{b}^r)}{q(c_i^*, \mathbf{b}^{s*}, \mathbf{b}^{r*})}\frac{P(\mathbf{c}^*,\mathbf{b}^{s*},\mathbf{b}^{r*})}{P(\mathbf{c},\mathbf{b}^{s},\mathbf{b}^{r})}\right)$$

In our case, the c terms cancel, and we have

$$\min\left(1, \frac{\prod_{j\in \mathcal{M}^s} q(g_j^s) \prod_{k\in \mathcal{M}^r} q(g_j^r)}
{\prod_{j\in \mathcal{M}^s} q(g_j^{s*}) \prod_{k\in \mathcal{M}^r} q(g_j^{r*})}
\frac{\prod_i P(g_i^{s*}|g_{<i}^{s*}, h, z_{\leq i}) P(g_i^{r*}|g_{<i}^{r*}, h,z_{\leq i})}
{\prod_i P(g_i^{s}|g_{<i}^{s}, h,z_{\leq i}) P(g_i^{r}|g_{<i}^{r}, h,z_{\leq i})}\right)
$$
where

$$P(g_j^s = k|g_{<j}^s, h, z_{\leq i}) \propto \begin{cases} 
f_2(d_{jk})  & k<j, z^*_i=z^*_k \\
\tau h_{s_j} & k=j\\
0 & z_j \neq z_k \end{cases}$$


Note this looks really similar to $q(g_j^s)$ above!! But it's not the same... because we are not conditioning on $s_i$. We do \textit{not} have zero probability for the case where $s_i\neq s_k$ -- so the normalizing constant will be different since we are summing over all pairs in the cluster, not just all pairs that are a match.

We can probably cancel some of the terms down here... but for now, I'd say let's not.


\subsection{Sampling the tables}
Conditioned on the cluster allocations $z_i$, we \textit{almost} have a hierarchical ddCRP as described in \cite{Ghosh2011} -- the only difference is that the top level of the hierarchy is a Pitman-Yor process, not a Dirichlet process. I will describe for sender-tables; receiver-tables are sampled analogously.

We consider the $i$th sender. It sender-follows $j$ with probability

$$P(g_i^s = j|g_{-i}^s, h, e) \propto \begin{cases} f_2(d_{ij} )P(s_i|g_i^s=j) & z_i=z_j, j<i\\
\tau P(s_i|g_i=i) & i=j\\
0 & z_i\neq z_j\end{cases}$$

Now, the likelihood is binary for an existing table (either the table ``serves'' $s_i$ or it doesn't), so this reduces to

\begin{equation}P(g_i^s = j|g_{-i}^s, h, e) \propto \begin{cases} f_2(d_{ij} )& z_i=z_j, j<i, s_i=s_j\\
\tau h_{s_i} & i=j\\
0 & z_i\neq z_j\\
0 & s_i \neq s_j\end{cases}\end{equation}






%Sampling the tables given the clusters is pretty straightforward. But, I'm leaving it for tomorrow so I have fresh eyes. 

\subsection{Sampling the $h$}

The $g_i^s$ and $g_i^r$ define tables $b_i^s$, $b_i^r$. Let $\eta_v$ be the total number of tables (sender and recipient) associated with vertex $v$. Then, assuming we have $V$ distinct vertices in our graph, we have

$$(h_1, \dots, h_V, h_+) \sim \mbox{Dirichlet} (\eta_1 - \sigma, \dots, \eta_V - \sigma, \gamma + V \sigma)$$

(see Corollary 20 of \cite{Pitman1996})
% $$q(c^{*}|c) = \big(P(c^{*}_i) + L(c^{*}_i|X)\big)-\big(P(c_i) + L(c_i|X)\big)$$

\begin{algorithm}[tb]
	\begin{algorithmic}[1]
	\STATE $c_i$ represents who the $i$-th edge is following: $(z_i, g_i^s,g_i^r)$
	\STATE Initialize $c_i$, $g_i^s$, $g_i^r$ for each edge $i$, assign the cluster indicators $z_i$ based on the $c_i$, assign the table indicators $b_i^s$, $b_i^r$ based on $g_i^s$, $g_i^r$.
    \STATE Calculate $f_1(d_{ij})$ and $f_2(d_{ij})$ for every $i, j \in 1, \dots, N$ 
 	\FOR {$t \in \{1,\ldots,MAXIT\}$}
 	\FOR{$i \in \{1, \dots, N\}$} 
 	\STATE \COMMENT{--Sampling the clusters--}
 	\STATE $\mathbf{c}^\circ \leftarrow \mathbf{c}$, $\mathbf{z}^\circ \leftarrow \mathbf{z}$, $\mathbf{g}^{s/r\circ} \leftarrow \mathbf{g}^{s/r} $
 	\STATE $c_i^{\circ} = i$
 	\STATE update all $z_i^{\circ}$ to be consistent with $c_i^{\circ}$
 	\STATE $\mathcal{M}^s = \{j: z_j^{\circ} \neq z_{g^s_j}^{\circ}\}$, $\mathcal{M}^r = \{j: z_j^{\circ} \neq z_{g^r_j}^{\circ}\}$
    % \FORALL{$j \in \mathcal{M}^{(s/r)}$}
    % \STATE $g_j^{(s/r)o} = j$
    % \ENDFOR
    % \FORALL{$j \not\in \mathcal{M}^{(s/r)}$}
    % \STATE $g_j^{(s/r)o} = g_j^{(s/r)}$
    % \ENDFOR
 	\STATE sample a proposal $c_i^*,g^{s*},g^{r*} \propto q(c_i, g^s, g^r) = q(c_i)\prod_{j\in \mathcal{M}^s} q(g_j^s) \prod_{k\in \mathcal{M}^r} q(g_k^r)$
 	\STATE sample $c_i^* \sim q(c_i), q(c_i=k) = \begin{cases} \frac{f_1(d_{ik})}{\sum_j f_1(d_{ij}) + \alpha} & k<i\\ \frac{\alpha}{\sum_j f_1(d_{ij}) + \alpha} & k=i\end{cases}$, then update $z^*$ from $c^*$
 	\FORALL{$j \in \mathcal{M}^{s/r}$}
 	\STATE sample $g_j^{*s/r} \sim q(g_j^{s/r})$ where
 	\STATE $q(g_j^s = k) := P(g_j^s = k | z_{\leq j}, g_{<j}^s, s_j) = \begin{cases} 
\frac{f_2(d_{jk})}{\sum_{l:z_l=z_k,s_l=s_k} f_2(d_{jl}) + \tau h_{s_j}}  & k<j, z^*_j=z^*_k, s_j = s_k \\
\frac{\tau h_{s_j}}{\sum_{l:z_l=z_k,s_l=s_k} f_2(d_{jl}) + \tau h_{s_j}} & k=j\\
0 & z^*_j\neq z^*_k\\
0 & s_j \neq s_k \end{cases}$
 	\ENDFOR
    \STATE compute acceptance ratio $a(c^*,c) = \min \bigg(1, \frac{q(c_i,b^s,b^r)}{q(c^*_i,b^{*s},b^{*r}} \frac{P(c^*_i,b^{*s},b^{*r})}{P(c_i,b^s,b^r)}  \bigg)$
    \STATE $a(c^*,c)=
    \min\left(1, \frac{\prod_{j\in \mathcal{M}^s} q(g_j^s) \prod_{k\in \mathcal{M}^r} q(g_j^r)}
{\prod_{j\in \mathcal{M}^s} q(g_j^{s*}) \prod_{k\in \mathcal{M}^r} q(g_j^{r*})}
\frac{\prod_i P(g_i^{s*}|g_{<i}^{s*}, h, z_{\leq i}) P(g_i^{r*}|g_{<i}^{r*}, h,z_{\leq i})}
{\prod_i P(g_i^{s}|g_{<i}^{s}, h,z_{\leq i}) P(g_i^{r}|g_{<i}^{r}, h,z_{\leq i})}\right)$
    \STATE where $P(g_j^s = k | z_{\leq j}, g_{<j}^s) = \begin{cases} 
\frac{f_2(d_{jk})}{\sum_{l:z_l=z_k} f_2(d_{jl}) + \tau }  & k<j, z_j=z_k\\
\frac{\tau h_{s_j}}{\sum_{l:z_l=z_k} f_2(d_{jl}) + \tau } & k=j\\
0 & z_j\neq z_k \end{cases}$
    \IF{rand < $a(c^*,c)$}
    \STATE accept new state
    \ENDIF
 	\STATE \COMMENT{--Sampling the tables--}
 	\STATE sample $g_i^{s/r} \sim P(g_i^{s/r}=j|g^{s/r}_{-i},h , e) = \begin{cases} 
\frac{f_2(d_{ij})}{\sum_{l:z_l=z_j,s_l=s_j} f_2(d_{il}) + \tau h_{s_i}}  & j<i, z_i=z_j, s_i = s_j \\
\frac{\tau h_{s_i}}{\sum_{l:z_l=z_j,s_l=s_j} f_2(d_{il}) + \tau h_{s_i}} & j=i\\
0 & z_i\neq z_j\\
0 & s_i \neq s_j \end{cases}$ 
	\ENDFOR %loop of edges in launch set
 	\STATE \COMMENT{--Sampling the $h$--}
 	\FOR{$v \in V$}
 	\STATE $\eta_v = \sum_{i}\mathbbm{1}{(s_i=v,g_i^s=i)}+\mathbbm{1}{(r_i=v,g_i^r=i)}$ 
 	\STATE sample $h_v \sim \text{Dir}(\eta_1-\sigma,\ldots, \eta_V-\sigma, \gamma+V\sigma)$
 	\ENDFOR %loop over vertices for h
 
 	
 	\ENDFOR % loop of iteration

% 		    \STATE Record $q(c_i^*)$ and $q(c_i)$

% 		    \FOR{$j \in \{1, \dots, N\}$}
% 	        	\IF{$z_j = z_i$ \sinead{If they were in the same cluster before the proposal}}
% 		            \IF{$z_j^* \neq z_{g_i^s}^*$ \sinead{If the person they are sender-following isn't in the same cluster after the proposal}}
% 		                \STATE $\mathcal{M}^s \leftarrow \mathcal{M}^s \cup j$
% 		            \ENDIF
% 		            \IF{$z_j^* \neq z_{g_i^r}^*$ \sinead{If the person they are receiver-following isn't in the same cluster after the proposal}}
% 		                \STATE $\mathcal{M}^r \leftarrow \mathcal{M}^r \cup j$
% 		            \ENDIF
% 		        \ENDIF
% 		    \ENDFOR
% 		    \FOR{$j \in \mathcal{M}^s$ \sinead{Propose new tables for anyone who's table-following someone who is now in a different clusters}}
% 		        \STATE Propose $g_j^{s*} \sim q(g_j^s)$, where $$q(g_j^s) \propto \begin{cases}f_2(d_{jk}) & k<j, z^*_k = z^*j \\
% 		        \tau h_{s_j} & k=j\\
% 		        0 & z^*_k \neq z^*j
% 		        \end{cases}$$
% 		        \sinead{We will add in details of how to sample the $h$ later... this is analogous to the $h$'s in the very old code}
% 		    \ENDFOR
% 		    \FOR{$j \in \mathcal{M}^r$}
% 		        \STATE Propose $g_j^{r*} \sim q(g_j^r)$, where $$q(g_j^r) \propto \begin{cases}f_2(d_{jk}) & k<j, z^*_k = z^*j \\
% 		        \tau h_{r_j} & k=j\\
% 		        0 & z^*_k \neq z^*j
% 		        \end{cases}$$
% 		    \ENDFOR
% 		    \STATE Record the $q(g_j^{s*})$ for $j\in \mathcal{M}^s$ and $q(g_j^{r*})$ for $j\in\mathcal{M}^r$ for the proposed state
% 		    \STATE $q(c^*, b^{s*}, b^{r*}) = q(c_i^*)\prod_{j\in \mathcal{M}^s}q(g_j^{s*})\prod_{k\in \mathcal{M}^r}q(g_k^{r*})  $
% 		    \STATE Calculate $q(g_j^{s})$f or $j\in \mathcal{M}^s$ and $q(g_j^{r})$ for $j\in\mathcal{M}^r$ for the current state
% 		    \STATE $q(c, b^{s}, b^{r}) = q(c_i)\prod_{j\in \mathcal{M}^s}q(g_j^{s*})\prod_{k\in \mathcal{M}^r}q(g_k^{r*})  $
% 		    %\STATE Accept new state with probability $\min(1, \frac{q(c, b^s, b^r)}{q(c, b^{s*}, b^{r*})}$
%         \ENDFOR
%     \ENDFOR
		
	\end{algorithmic}
	\caption{MH}
	\label{alg:modified}
\end{algorithm}

\begin{algorithm}[th]
	\begin{algorithmic}[1]
	\STATE initialize $c_i$ uniformly at random from $\{1,\ldots,N\}$ for each edge $i$
	\FOR {$t \in \{1,\ldots,T\}$}
		\FOR {$i \in \{1,\ldots,N\}$}
		\FOR {$j \in \{1,\ldots,i-1\}$}
		    \STATE compute $f_{d_{ij}}$ \qquad \COMMENT{For the prior}
		\ENDFOR
		\STATE sample $z_i \propto \begin{cases} f_1(d_{ij})-\sigma \quad & j < i \\ \alpha+K\sigma \quad & j = i \end{cases}$
		\STATE $P(c^{*}_i) = \log p(z_i)$
		\IF{$z_i< K$}
		\STATE sample $b_i^{*(s/r)}|z_i \propto H = \begin{cases} \sum_{j:z_j=z_i}\frac{f_2(d_{ij})}{\sum_{j:z_j =z_i}f_1(d_{ij})+\tau} + \big(\frac{\tau}{\sum_{j:z_j =z_i}f_1(d_{ij})+\tau}\frac{t^{(s/r)}_i}{\sum_{l}t^{(s)}_l+t^{(r)}_l+\gamma} \big) \quad &t^{(s/r)}_i>0 \\ \frac{\tau}{\sum_{j:z_j =z_i}f_1(d_{ij})+\tau}\frac{\gamma}{\sum_{l}t^{(s)}_l+t^{(r)}_l+\gamma} \quad &t^{(s/r)}=0 \end{cases}$
		\ELSE
		\STATE sample $b_i^{*(s/r)}|z_i \propto H = \begin{cases} \frac{t^{(s/r)}_i}{\sum_{l}t^{(s)}_l+t^{(r)}_l+\gamma} \quad &t^{(s/r)}_i>0 \\ \frac{\gamma}{\sum_{l}t^{(s)}_l+t^{(r)}_l+\gamma} \quad &t^{(s/r)}=0 \end{cases}$
		\ENDIF
		\STATE $L(c^*_i|X) = \log p(b_i^{*(s)})+ \log p(b_i^{*(r)})$
		\STATE proposal = $q(c^{*}|c) = \big(P(c^{*}_i) + L(c^{*}_i|X)\big)-\big(P(c_i) + L(c_i|X)\big)$
		\STATE $a(c^{*},c) = \min(1, e^{q(c^{*}|c)})$
		\IF{rand < a}
		\STATE accept the proposal $c^{*}$
		\ELSE
		\STATE reject the proposal
		\ENDIF
		\ENDFOR
		\STATE \COMMENT{split-merge}
		\STATE pick $i$ and $j$ uniformly at random  
		\STATE $S$ is the set of observations, $k \in \{1,\ldots,n\}$ for which $k \neq i, k \neq j$ and $z_k=z_i  \OR z_k=z_j$
		\IF{$z_i = z_j$}
		\STATE $c^{*}=c^{split}$
		\STATE set $c_i^{split}$ to a new component such that $c_i^{split} \not\in \{c_1,\ldots,c_n\}$
		\STATE set $c_j^{split}=c_j$
		\STATE sample $b^{split (s/r)}_i, b^{split (s/r)}_j \propto H$ 
		\FOR{$k \in S$}
		\STATE $c_k^{split} = $ randomly choose $c_i^{split} \OR c_j^{split}$
		\STATE sample $b^{split (s/r)}_k \propto H$ 
		\ENDFOR
		\STATE compute prior $P(c^{split})$ and the likelihood of this clustering $L(c^{split}|X)$ just for changed clusters
		\STATE $a(c^{split},c) = \min\bigg(1, \frac{1}{\big(\frac{1}{2}\big)^{n_{c_i^{split}}+n_{c_j^{split}}-2}}\frac{P(c^{split})L(c^{split}|X)}{P(c)L(c|X)}\bigg)$
		\ELSE
	    \STATE $c^{*}=c^{merge}$
		\STATE set $c_i^{merge} = c_j$
		\STATE set $c_j^{merge}=c_j$
		\STATE sample $b^{merge (s/r)}_i, b^{split (s/r)}_j \propto H$ 
		\FOR{$k \in S$}
		\STATE $c_k^{merge} = c_j$
		\STATE sample $b^{merge (s/r)}_k \propto H$ 
        \ENDFOR
        \STATE compute prior $P(c^{merge})$ and the likelihood of this clustering $L(c^{merge}|X)$ just for changed clusters
		\STATE $a(c^{merge},c) = \min\bigg(1, \big(\frac{1}{2}\big)^{n_{c_i}+n_{c_j}-2}\frac{P(c^{merge})L(c^{merge}|X)}{P(c)L(c|X)}\bigg)$
        \ENDIF
        \STATE accept/reject $c^{*}$ based on the acceptance ratio $a(c^{*},c)$
	\ENDFOR
		
	\end{algorithmic}
	\caption{MH}
	\label{alg:ll}
\end{algorithm}







\iffalse
\begin{table*}[ht]
\parbox{\textwidth}{
\caption{\small{AP@10}\vspace{-.2cm}}
\centering
\scriptsize
\resizebox{1\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|}
	\toprule
	Method & \alg & MDND & DRGPM & DPGM & DGPPF\\ 
	\midrule
	\textsc{CollegeMsg} & \textbf{0.466$$\pm$$0.030} & 0.267$$\pm$$0.132 & 0.118$$\pm$$0.105  & 0.037$$\pm$$0.007 & 0.052$$\pm$$0.016 \\
	\textsc{Email-Eu}  & \textbf{0.390$$\pm$$0.052} & 0.238$$\pm$$0.101 & 0.330$$\pm$$0.124 & 0.308$$\pm$$0.110 & 0.199$$\pm$$0.099\\
	\textsc{SocialEv} & \textbf{0.586$$\pm$$0.338}  & 0.179$$\pm$$0.104 & 0.001$$\pm$$0.000 & 0.033$$\pm$$0.008 & 0.008$$\pm$$0.003 \\
	\textsc{DBLP} & \textbf{0.493$$\pm$$0.274} & 0.205$$\pm$$0.039 & 0.388$$\pm$$0.263 & 0.451$$\pm$$0.228 & 0.374$$\pm$$0.204\\
	\hline
\end{tabular}
}\label{tbl:hitall}\vspace{5mm}
}
\hfill
\parbox{\textwidth}{
\caption{\small{AP@20}\vspace{-.2cm}}
\centering
\scriptsize
\resizebox{1\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|}
	\toprule
	Method & \alg & MDND & DRGPM & DPGM & DGPPF\\ 
	\midrule
	\textsc{CollegeMsg} & \textbf{0.504$$\pm$$0.033} & 0.295$$\pm$$0.118 & 0.091$$\pm$$0.060  & 0.071$$\pm$$0.064 & 0.085$$\pm$$0.070 \\
	\textsc{Email-Eu}  & 0.452$$\pm$$0.012 & 0.227$$\pm$$0.097 & \textbf{0.464$$\pm$$0.112} & 0.451$$\pm$$0.091 & 0.380$$\pm$$0.087 \\
	\textsc{SocialEv} & \textbf{0.515$$\pm$$0.232}  & 0.162$$\pm$$0.239 & 0.008$$\pm$$0.003 & 0.011$$\pm$$0.009 & 0.014$$\pm$$0.006 \\
	\textsc{DBLP} & 0.496$$\pm$$0.143 & 0.118$$\pm$$0.019 & 0.459$$\pm$$0.254 & \textbf{0.516$$\pm$$0.229} & 0.485$$\pm$$0.197\\
	\hline
\end{tabular}}
\label{tbl:apall}\vspace{5mm}
}
\hfill
\parbox{\textwidth}{
\caption{\small{AP@50}\vspace{-.2cm}}
\centering
\scriptsize
\resizebox{.9\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|}
	\toprule
	Method & \alg & MDND & DRGPM & DPGM & DGPPF\\ 
	\midrule
	\textsc{CollegeMsg} & \textbf{0.516$$\pm$$0.026} & 0.321$$\pm$$0.065  & 0.085$$\pm$$0.052  & 0.067$$\pm$$0.061 & 0.069$$\pm$$0.065 \\
	\textsc{Email-Eu}  & \textbf{0.585$$\pm$$0.036} & 0.318$$\pm$$0.125 & 0.494$$\pm$$0.117 & 0.490$$\pm$$0.104 & 0.451$$\pm$$0.091\\
	\textsc{SocialEv} & \textbf{0.423$$\pm$$0.151}  & 0.253$$\pm$$0.169 & 0.009$$\pm$$0.004 & 0.024$$\pm$$0.010 & 0.021$$\pm$$0.006 \\
	\textsc{DBLP} & 0.492$$\pm$$0.111 & 0.241$$\pm$$0.012 & 0.451$$\pm$$0.234 & \textbf{0.498$$\pm$$0.208} & 0.476$$\pm$$0.181\\
	\hline
\end{tabular}}
\label{tbl:hitmapk100}\vspace{5mm}
}
\hfill
\parbox{\textwidth}{
\caption{\small{AP@$\mathtt{k}$ of three decay functions}\vspace{-2mm}}
\centering
\scriptsize
\resizebox{1\textwidth}{!}{
\begin{tabular}{|c|ccc|ccc|ccc|}
	\toprule
	& \multicolumn{3}{|c|}{\alg-\textsc{Window}} &\multicolumn{3}{|c|}{\alg-\textsc{Logistic}} & \multicolumn{3}{|c|}{\alg-\textsc{Exponential}} \\ 
	\midrule
	\textit{MAP@$\mathtt{k}$} & @10 & @20 & @50& @10 & @20 & @50 & @10 & @20 & @50  \\ 
	\midrule
	\textsc{CollegeMsg} & \textbf{0.47$$\pm$$0.03} & \textbf{0.50$$\pm$$0.03} & \textbf{0.52$$\pm$$0.03} & 0.46$$\pm$$0.15 & 0.50$$\pm$$0.09 & 0.51$$\pm$$0.14 & 0.46$$\pm$$0.11 & 0.48$$\pm$$0.11 & 0.49$$\pm$$0.15  \\
	\textsc{Email-Eu}   & 0.25$$\pm$$0.04 & 0.39$$\pm$$0.01 & 0.46$$\pm$$0.09 & 0.33$$\pm$$0.08 & 0.43$$\pm$$0.04 & 0.50$$\pm$$0.10 & \textbf{0.39$$\pm$$0.05} & \textbf{0.45$$\pm$$0.01} & \textbf{0.50$$\pm$$0.04} \\
	\textsc{SocialEv}   & 0.34$$\pm$$0.16 & 0.32$$\pm$$0.02 & 0.28$$\pm$$0.03 & 0.50$$\pm$$0.36 & 0.51$$\pm$$0.30 & \textbf{0.49$$\pm$$0.27} & \textbf{0.59$$\pm$$0.34} &\textbf{0.51$$\pm$$0.23} & 0.42$$\pm$$0.15  \\
	\textsc{DBLP}       & 0.39$$\pm$$0.11 & 0.42$$\pm$$0.07 & 0.45$$\pm$$0.05 & 0.46$$\pm$$0.14 & 0.40$$\pm$$0.07 & 0.49$$\pm$$0.05 & \textbf{0.49$$\pm$$0.27} & \textbf{0.50$$\pm$$0.14} & \textbf{0.49$$\pm$$0.11} \\
	\hline
\end{tabular}
}\label{tbl:decay_Maps}
}
\end{table*}

\fi


% \begin{table*}[t]
% \caption{Map@$\mathtt{k}$ of three decay functions.}
% \centering
% \scriptsize
% \begin{tabular}{|c|ccc|ccc|ccc|}
% 	\toprule
% 	& \multicolumn{3}{|c|}{\alg-\textsc{Window}} &\multicolumn{3}{|c|}{\alg-\textsc{Logistic}} & \multicolumn{3}{|c|}{\alg-\textsc{Exponential}} \\ 
% 	\midrule
% 	\textit{MAP@$\mathtt{k}$} & @10 & @20 & @50& @10 & @20 & @50 & @10 & @20 & @50  \\ 
% 	\midrule
% 	\textsc{CollegeMsg} & \textbf{0.47$$\pm$$0.03} & \textbf{0.50$$\pm$$0.03} & \textbf{0.52$$\pm$$0.03} & 0.46$$\pm$$0.15 & 0.50$$\pm$$0.09 & 0.51$$\pm$$0.14 & 0.46$$\pm$$0.11 & 0.48$$\pm$$0.11 & 0.49$$\pm$$0.15  \\
% 	\textsc{Email-Eu}   & 0.25$$\pm$$0.04 & 0.39$$\pm$$0.014 & 0.46$$\pm$$0.09 & 0.33$$\pm$$0.08 & 0.43$$\pm$$0.04 & 0.500$$\pm$$0.10 & \textbf{0.39$$\pm$$0.05} & \textbf{0.45$$\pm$$0.01} & \textbf{0.50$$\pm$$0.04} \\
% 	\textsc{SocialEv}   & 0.34$$\pm$$0.16 & 0.32$$\pm$$0.02 & 0.28$$\pm$$0.03 & 0.50$$\pm$$0.36 & 0.51$$\pm$$0.30 & \textbf{0.49$$\pm$$0.27} & \textbf{0.59$$\pm$$0.34} &\textbf{0.51$$\pm$$0.23} & 0.42$$\pm$$0.15  \\
% 	\textsc{DBLP}       & 0.39$$\pm$$0.11 & 0.42$$\pm$$0.07 & 0.45$$\pm$$0.05 & 0.46$$\pm$$0.14 & 0.40$$\pm$$0.07 & 0.49$$\pm$$0.05 & \textbf{0.49$$\pm$$0.27} & \textbf{0.50$$\pm$$0.14} & \textbf{0.49$$\pm$$0.11} \\
% 	\hline
% \end{tabular}\label{tbl:decay_Maps}
% \end{table*}


% \begin{table*}\caption{Map@$\mathtt{k}$ of three decay functions.}
% \centering
% \scriptsize
% \begin{tabular}{|c|ccc|ccc|ccc|}
% 	\toprule
% 	& \multicolumn{3}{|c|}{\alg-\textsc{Window}} &\multicolumn{3}{|c|}{\alg-\textsc{Logistic}} & \multicolumn{3}{|c|}{\alg-\textsc{Exponential}} \\ 
% 	\midrule
% 	\textit{MAP@$\mathtt{k}$} & @10 & @20 & @50& @10 & @20 & @50 & @10 & @20 & @50  \\ 
% 	\midrule
% 	\textsc{CollegeMsg} & \textbf{0.466$$\pm$$0.030} & \textbf{0.504$$\pm$$0.033} & \textbf{0.462$$\pm$$0.151} & 0.501$$\pm$$0.090 & 0.511$$\pm$$0.144 & 0.460$$\pm$$0.111 & 0.480$$\pm$$0.106 & 0.491$$\pm$$0.146 &  \\
% 	\textsc{Email-Eu}   & 0.248$$\pm$$0.039 & 0.393$$\pm$$0.014 & 0.460$$\pm$$0.087 & 0.334$$\pm$$0.085 & 0.427$$\pm$$0.041 & 0.499$$\pm$$0.097 & \textbf{0.390$$\pm$$0.052} & \textbf{0.452$$\pm$$0.012} & \textbf{0.505$$\pm$$0.036} \\
% 	\textsc{SocialEv}   & 0.344$$\pm$$0.165 & 0.321$$\pm$$0.024 & 0.279$$\pm$$0.034 & 0.505$$\pm$$0.356 & 0.510$$\pm$$0.301 & \textbf{0.488$$\pm$$0.270} & \textbf{0.586$$\pm$$0.338} & 0.423$$\pm$$0.151 &  \\
% 	\textsc{DBLP}       & 0.391$$\pm$$0.106 & 0.423$$\pm$$0.067 & 0.448$$\pm$$0.052 & 0.463$$\pm$$0.143 & 0.400$$\pm$$0.068 & 0.487$$\pm$$0.052 & \textbf{0.493$$\pm$$0.274} & \textbf{0.496$$\pm$$0.143} & \textbf{0.492$$\pm$$0.111} \\
% 	\hline
% \end{tabular}\label{tbl:decay_Maps}
% \end{table*}


\begin{algorithm}[tb]
	\begin{algorithmic}[1]
	\STATE initialize $c_i$ uniformly at random from $\{1,\ldots,N\}$ for each edge $i$
	\FOR {$t \in \{1,\ldots,T\}$}
		\FOR {$i \in \{1,\ldots,N\}$}
		\FOR {$j \in \{1,\ldots,i-1\}$}
		    \STATE compute $f_{d_{ij}}$ \qquad \COMMENT{For the prior}
		\ENDFOR
		\STATE sample $z_i \propto \begin{cases} f_1(d_{ij})-\sigma \quad & j < i \\ \alpha+K\sigma \quad & j = i \end{cases}$
		\STATE $P(c^{*}_i) = \log p(z_i)$
		\IF{$z_i< K$}
		\STATE sample $b^{*}_i^{(s/r)}|z_i \propto H = \begin{cases} \sum_{j:z_j=z_i}\frac{f_2(d_{ij})}{\sum_{j:z_j =z_i}f_1(d_{ij})+\tau} + \big(\frac{\tau}{\sum_{j:z_j =z_i}f_1(d_{ij})+\tau}\frac{t^{(s/r)}_i}{\sum_{l}t^{(s)}_l+t^{(r)}_l+\gamma} \big) \quad &t^{(s/r)}_i>0 \\ \frac{\tau}{\sum_{j:z_j =z_i}f_1(d_{ij})+\tau}\frac{\gamma}{\sum_{l}t^{(s)}_l+t^{(r)}_l+\gamma} \quad &t^{(s/r)}=0 \end{cases}$
		\ELSE
		\STATE sample $b^{*}_i^{(s/r)}|z_i \propto H = \begin{cases} \frac{t^{(s/r)}_i}{\sum_{l}t^{(s)}_l+t^{(r)}_l+\gamma} \quad &t^{(s/r)}_i>0 \\ \frac{\gamma}{\sum_{l}t^{(s)}_l+t^{(r)}_l+\gamma} \quad &t^{(s/r)}=0 \end{cases}$
		\ENDIF
		\STATE $L(c^{*}_i|X) = \log p(b^{*}_i^{(s)})+ \log p(b^{*}_i^{(r)})$
		\STATE proposal = $q(c^{*}|c) = \big(P(c^{*}_i) + L(c^{*}_i|X)\big)-\big(P(c_i) + L(c_i|X)\big)$
		\STATE $a(c^{*},c) = \min(1, e^{q(c^{*}|c)})$
		\IF{rand < a}
		\STATE accept the proposal $c^{*}$
		\ELSE
		\STATE reject the proposal
		\ENDIF
		\ENDFOR
		\STATE \COMMENT{split-merge}
		\STATE pick $i$ and $j$ uniformly at random  
		\STATE $S$ is the set of observations, $k \in \{1,\ldots,n\}$ for which $k \neq i, k \neq j$ and $z_k=z_i  \OR z_k=z_j$
		\IF{$z_i = z_j$}
		\STATE $c^{*}=c^{split}$
		\STATE set $c_i^{split}$ to a new component such that $c_i^{split} \not\in \{c_1,\ldots,c_n\}$
		\STATE set $c_j^{split}=c_j$
		\STATE sample $b^{split (s/r)}_i, b^{split (s/r)}_j \propto H$ 
		\FOR{$k \in S$}
		\STATE $c_k^{split} = $ randomly choose $c_i^{split} \OR c_j^{split}$
		\STATE sample $b^{split (s/r)}_k \propto H$ 
		\ENDFOR
		\STATE compute prior $P(c^{split})$ and the likelihood of this clustering $L(c^{split}|X)$ just for changed clusters
		\STATE $a(c^{split},c) = \min\bigg(1, \frac{1}{\big(\frac{1}{2}\big)^{n_{c_i^{split}}+n_{c_j^{split}}-2}}\frac{P(c^{split})L(c^{split}|X)}{P(c)L(c|X)}\bigg)$
		\ELSE
	    \STATE $c^{*}=c^{merge}$
		\STATE set $c_i^{merge} = c_j$
		\STATE set $c_j^{merge}=c_j$
		\STATE sample $b^{merge (s/r)}_i, b^{split (s/r)}_j \propto H$ 
		\FOR{$k \in S$}
		\STATE $c_k^{merge} = c_j$
		\STATE sample $b^{merge (s/r)}_k \propto H$ 
        \ENDFOR
        \STATE compute prior $P(c^{merge})$ and the likelihood of this clustering $L(c^{merge}|X)$ just for changed clusters
		\STATE $a(c^{merge},c) = \min\bigg(1, \big(\frac{1}{2}\big)^{n_{c_i}+n_{c_j}-2}\frac{P(c^{merge})L(c^{merge}|X)}{P(c)L(c|X)}\bigg)$
        \ENDIF
        \STATE accept/reject $c^{*}$ based on the acceptance ratio $a(c^{*},c)$
% 		\STATE sample $z_n \propto \begin{cases} f(d_{ij}) \quad & j \neq n \\ \alpha \quad & j = n \end{cases}$ 
% 		\STATE sample $b_n^{s/r}|z_n \propto H $
% 		
% 		
		
	\ENDFOR
		
	\end{algorithmic}
	\caption{MH}
	\label{alg:ll}
\end{algorithm}


